DSEffi-Bench: Demystifying Large Language Models' Capability in Efficient Data Science Code Generation

Current data science (DS) code generation benchmarks equate correctness with quality, overlooking execution time differences that span orders of magnitude between correct solutions. We introduce DSEffi-Bench, the first benchmark specifically targeting execution efficiency in LLM-generated DS code, comprising 1,000 instances across 10+ DS libraries with stress-testing harnesses and human-validated references. Evaluating 16 models across 3 tiers, we find that correctness alone fails to characterize efficiency: GPT-5.4 leads in correctness (Pass, 66.9\%) but its efficiency score (B$|$P, 71.7\%) nearly matches GPT-5.4-mini (71.6\%), which solves 47 fewer tasks; Kimi-K2.5 ranks lowest in correctness among frontier models (40.2\%) yet achieves the highest efficiency score (73.6\%) across all 16 models. A human-annotated five-category taxonomy reveals that 79.1\% of efficiency deficits extend beyond algorithmic complexity to domain-specific root causes, with distinct failure profiles across model tiers and libraries. Two exploratory experiments provide initial evidence that these diagnostics can guide improvement, yielding up to +14.7\% efficiency gains via taxonomy-guided optimization and approaching Claude-Opus-4.6 Best@3 in efficiency at 13.0$\times$ lower cost via library-conditioned routing.

==> Table/pairwise_winrate_matrix.tex <==
GPT-5.4 & --- & 28.3 & 34.1 & 42.5 & 43.7 & 55.5 & 27.7 & 47.6 & 38.2 & 54.0 & 56.2 & 55.1 & 67.3 & 58.4 & 62.4 & 64.4 \\
5.4-mini & 26.0 & --- & 35.5 & 39.2 & 39.2 & 52.4 & 24.5 & 46.6 & 38.2 & 52.0 & 51.2 & 50.6 & 63.8 & 58.2 & 57.0 & 63.6 \\
Opus-4.6 & 31.6 & 31.6 & --- & 33.7 & 38.9 & 53.3 & 29.6 & 46.6 & 33.1 & 50.5 & 53.8 & 53.7 & 62.6 & 51.4 & 60.7 & 63.5 \\
Sonnet-4.6 & 26.6 & 27.8 & 23.4 & --- & 31.0 & 44.7 & 23.6 & 40.1 & 29.6 & 46.6 & 45.9 & 46.0 & 56.3 & 48.4 & 56.1 & 60.9 \\
\midrule
V4-Flash & 23.0 & 26.0 & 26.9 & 30.6 & --- & 38.9 & 17.4 & 35.1 & 24.4 & 41.9 & 42.9 & 42.7 & 49.8 & 44.8 & 51.4 & 55.2 \\
V3.2 & 19.2 & 17.5 & 22.2 & 25.1 & 26.4 & --- & 17.4 & 32.8 & 22.7 & 34.3 & 39.2 & 38.3 & 46.7 & 44.3 & 45.5 & 52.8 \\
Kimi & 30.1 & 34.4 & 33.0 & 39.5 & 34.8 & 53.2 & --- & 46.8 & 38.4 & 52.7 & 53.9 & 53.2 & 61.0 & 48.7 & 54.7 & 66.0 \\
MiniMax & 20.7 & 24.4 & 23.8 & 28.9 & 25.6 & 38.6 & 16.7 & --- & 19.7 & 38.8 & 42.1 & 37.4 & 51.7 & 43.8 & 46.2 & 57.4 \\
Qwen3.5 & 25.5 & 24.4 & 28.0 & 29.6 & 31.4 & 45.3 & 23.6 & 36.4 & --- & 44.0 & 46.8 & 46.4 & 57.1 & 46.5 & 62.2 & 62.3 \\
\midrule
QCoder-Nxt & 21.7 & 19.4 & 23.8 & 25.6 & 24.2 & 34.0 & 20.1 & 29.9 & 21.5 & --- & 36.4 & 38.7 & 46.7 & 38.1 & 50.0 & 49.6 \\
Devstrl-123 & 18.5 & 20.3 & 20.1 & 26.1 & 21.0 & 29.4 & 18.7 & 28.4 & 18.9 & 33.3 & --- & 34.7 & 41.2 & 35.5 & 39.8 & 47.8 \\
QC-32B & 25.0 & 25.9 & 28.5 & 26.8 & 28.1 & 37.5 & 22.0 & 33.5 & 23.8 & 32.8 & 31.4 & --- & 34.7 & 32.9 & 47.7 & 43.6 \\
QC-14B & 16.0 & 16.9 & 21.0 & 25.8 & 23.4 & 26.8 & 22.5 & 26.3 & 21.1 & 26.7 & 23.2 & 23.3 & --- & 25.1 & 36.3 & 36.7 \\
Codestrl-22 & 17.3 & 15.5 & 23.9 & 23.0 & 28.5 & 26.9 & 21.1 & 30.8 & 22.8 & 27.8 & 28.0 & 24.4 & 34.9 & --- & 24.5 & 34.8 \\
DS-33B & 17.4 & 20.1 & 15.6 & 22.7 & 18.1 & 30.6 & 18.9 & 26.4 & 20.5 & 21.0 & 26.8 & 18.0 & 29.2 & 26.6 & --- & 44.3 \\
DS-V2-Lite & 26.7 & 22.1 & 22.6 & 21.1 & 21.0 & 24.0 & 22.3 & 26.6 & 21.7 & 29.6 & 28.7 & 31.7 & 29.4 & 35.9 & 27.9 & --- \\

